Review-driven Personalized Preference Reasoning with Large Language Models for Recommendation

Recent advancements in Large Language Models (LLMs) have demonstrated exceptional performance across a wide range of tasks, generating significant interest in their application to recommendation systems. However, existing methods have not fully capitalized on the potential of LLMs, often constrained by limited input information or failing to fully utilize their advanced reasoning capabilities. To address these limitations, we introduce EXP3RT, a novel LLM-based recommender designed to leverage rich preference information contained in user and item reviews. EXP3RT is basically fine-tuned through distillation from a teacher LLM to perform three key tasks in order: EXP3RT first extracts and encapsulates essential subjective preferences from raw reviews, aggregates and summarizes them according to specific criteria to create user and item profiles. It then generates detailed step-by-step reasoning followed by predicted rating, i.e., reasoning-enhanced rating prediction, by considering both subjective and objective information from user/item profiles and item descriptions. This personalized preference reasoning from EXP3RT enhances rating prediction accuracy and also provides faithful and reasonable explanations for recommendation. Extensive experiments show that EXP3RT outperforms existing methods on both rating prediction and candidate item reranking for top-k recommendation, while significantly enhancing the explainability of recommendation systems.

==> 041RatingPredTable.tex <==
\begin{table}[t]
\centering
\caption{Performance for rating prediction. The best and second-best results are highlighted in bold and underlined.}
\label{tbl:rating_prediction_table}
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{lUUUU}
\toprule
\multirow{2.5}{*}{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{IMDB}} & \multicolumn{2}{c}{\textbf{Amazon-book}} \\ \cmidrule(lr){2-3}\cmidrule(lr){4-5}
 & \textbf{RMSE} & \textbf{MAE} & \textbf{RMSE} & \textbf{MAE} \\ \midrule

\mf & \underline{1.9530} & \underline{1.4771} &  \underline{0.6683} & 0.4572 \\
\mlp & 2.2562 & 1.7467 & 0.7020 & 0.5324 \\
\rgcl & 2.3143 & 1.8036  & 0.7562 & 0.6117 \\ \midrule
\pfive & 2.5471 & 1.8604 & 0.8868 & 0.4756 \\
\llmrec (\gptthree, ZS) & 2.4843 & 1.7559 & 0.8974 &  0.6356 \\
\llmrec (\gptthree, FS) & 2.2161 & 1.6223 & 0.7852 & \underline{0.4562} \\
\llmrec (\gptfour, ZS) & 2.1586 & 1.6261 & 0.9986 & 0.8331 \\
\llmrec (\gptfour, FS) & 2.1410 & 1.6334 & 0.8386 & 0.5004 \\
\proposed & \textbf{1.9122}* & \textbf{1.4691}* & \textbf{0.6508}* & \textbf{0.4297}* \\ \bottomrule

\end{tabular}
}
\end{table}

==> 044ColdStartTable.tex <==
\begin{table}[t]
\centering
\caption{Performance for rating prediction on warm-start, cold-start, and unseen users/items, Dataset: \amazon.}
\label{tbl:coldstart_table}
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2.5}{*}{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{Warm-start}} & \multicolumn{2}{c}{\textbf{Cold-start}} & \multicolumn{2}{c}{\textbf{Unseen}}\\ \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 & \textbf{RMSE} & \textbf{MAE} & \textbf{RMSE} & \textbf{MAE} & \textbf{RMSE} & \textbf{MAE} \\ \midrule

\mf & \underline{0.6663} & \underline{0.4588} & \underline{0.6769} & 0.4501 & - & -\\
\mlp & 0.6963 & 0.5280 & 0.7262 & 0.5519 & - & -\\
\rgcl & 0.7533 & 0.6109 & 0.7693 & 0.6154 & - & -\\ \midrule
\pfive & 0.8873 & 0.4810 & 0.8846 & 0.4508 & - & -\\
{\small \llmrec (3.5, ZS)} & 0.8910 & 0.6301 & 0.9260 & 0.6609 & 1.9732 & 1.6170 \\
{\small \llmrec (3.5, FS)} & 0.7888 & 0.4623 & 0.7688 & \underline{0.4286} & 1.7607 & 1.3000 \\
{\small \llmrec (4, ZS)} & 0.9941 & 0.8257 & 1.0187 & 0.8670 & 1.7139 & 1.3958 \\
{\small \llmrec (4, FS)} & 0.8370 & 0.5010 & 0.8460 & 0.4974 & 1.4993 & \textbf{1.0300}* \\
\proposed & \textbf{0.6572}* & \textbf{0.4369}*  & \textbf{0.6072}* & \textbf{0.3858}* & \textbf{1.4398}* & \underline{1.1192}\\ \bottomrule
% \pfive & - & - & - & - \\
% \gptthree(zero-shot) & 2.4843 & 1.7559 & - & - \\
% \gptthree(few-shot) & 2.2161 & 1.6223 & - & - \\ 
% \gptfour(zero-shot) & 2.1586 & 1.6261 & - & - \\
% \gptfour(few-shot) & 2.1410 & 1.6334 & - & - \\  
% \proposed & 1.9912 & 1.4767 & \textbf{0.6508} & \textbf{0.4297} \\ \bottomrule

\end{tabular}
}
\end{table}

==> 047Datasets.tex <==
\begin{table}[t]
\centering
\caption{Statistics of the datasets}
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Dataset} & \textbf{\#Users} & \textbf{\#Items} & \textbf{\#Interactions}  & \textbf{Density}\\
\midrule
\imdb & \ \ \ \ \ 859 & \ \ 1,155 & \ \ 19,124 & 0.0193 \\
\amazon & 10,761 & 10,084 & 118,705 & 0.0011 \\
\bottomrule
\end{tabular}
}
% \vspace{0.2cm}
\label{tbl:dataset_statistics}
\end{table}

==> 048ComponentAnalysis_additional.tex <==
To validate the performance using different LLM, we use the same prompts provided to \proposed, which corresponds to the third method in Table \ref{tbl:no_bias_reasoning}, but employing GPT-4 instead of GPT-3.5.
The result in Table \ref{tbl:no_bias_reasoning_additional} supports the necessity of fine-tuning in the recommendation domain and shows that knowledge distillation process improves a smaller LLM, enhancing both cost-efficiency and recommendation accuracy.
% While GPT-4 offers advanced capabilities, we choose GPT-3.5 as the teacher LLM for its ability to generate high-quality labeled data at a substantially lower computational cost, ensuring a balance between efficiency and effectiveness.


\begin{table}[H]
\centering
\caption{Validation with different LLM (*: $p$-value < 0.05).}
\label{tbl:no_bias_reasoning_additional}
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{cccQQQQ}
\toprule
\multirow{2.5}{*}{\textbf{Methods}} & \multirow{2.5}{*}{\textbf{R}} & \multirow{2.5}{*}{\textbf{B}} & \multicolumn{2}{c}{\textbf{IMDB}} & \multicolumn{2}{c}{\textbf{Amazon-book}} \\ \cmidrule(lr){4-5}\cmidrule(lr){6-7}
& & & \textbf{RMSE} & \textbf{MAE} & \textbf{RMSE} & \textbf{MAE} \\ \midrule
% \gptfour & \cmark & \cmark & 2.0688 & 1.6489 & 0.9038 & 0.6518 \\ \midrule
{\shortstack{\gptfour, ZS}} & \cmark & \cmark & 2.0628 & 1.5769 & 0.9120 & 0.5788 \\ \midrule

% \gptthree & \cmark & \cmark & 2.0688 & 1.6489 & 0.9038 & 0.6518 \\ \midrule
{\shortstack{\gptthree, ZS}} & \cmark & \cmark & 2.0688 & 1.6489 & 0.9038 & 0.6518 \\ \midrule

\proposed & \cmark & \cmark & \textbf{1.9122}* & \textbf{1.4691}* & \textbf{0.6508}* & \textbf{0.4297}* \\ \bottomrule
\end{tabular}
}
\end{table}

==> 080humaneval.tex <==
We evaluate the quality of the generated explanations by outsourcing a human evaluation, comparing the outputs of \proposed with those from other baseline models using Amazon Mechanical Turk (AMT).
% We show the interface for the evaluation in Figure .
We ask three human judges to compare the quality of explanation based on the following five criteria:
% \begin{itemize}
% [leftmargin=*,topsep=2pt,itemsep=2pt,parsep=0pt]
%     \item \textbf{Persuasiveness}: Which explanation is more persuasive in convincing the user to accept the recommendation?
%     \item \textbf{Reasonability}: Which explanation is more logical and reasonable?
%     \item \textbf{Scrutability}: Which explanation better helps the user understand their preferences for the item?
%     \item \textbf{Faithfulness}: Which explanation better reflects the actual content, features, or attributes of the recommended item?
%     \item \textbf{Overall}: Which explanation has a higher overall quality as a recommendation explanation?
% \end{itemize}
\textbf{Persuasiveness}, which measures how convincing the explanation is in making the user accept the recommendation; \textbf{Reasonability}, assessing the logical and reasonable nature of the explanation; 
\textbf{Scrutability}, determining how well the explanation helps the user understand their preferences for the item; \textbf{Faithfulness}, evaluating how accurately the explanation reflects the actual content, features, or attributes of the recommended item; and 
\textbf{Overall}, which judges the general quality of the explanation as a recommendation explanation.
% During each stage of voting, human judges are given \textbf{user/item profile}, item description and two explanation candidates and asked to judge which one is of a higher quality based on the above criteria.


==> 090dataset.tex <==
We evaluated \proposed on datasets with varying density levels since CF methods are more advantageous in higher density. 
For the {\imdb} dataset, we set higher density, which led to fewer interactions and limited recommendation diversity. 
% On the other hand, {\amazon} dataset is set to be lower density and attendant upon a broader range of scenarios, including cold and warm start and unseen cases. 
On the other hand, the {\amazon} dataset is set to have lower density, covering a broader range of scenarios such as cold-start, warm-start, and unseen cases.
\proposed performed well on both high and low-density datasets than CF methods, demonstrating its robustness.

==> 092efficiency.tex <==
% For computational efficiency, we conducted additional experiments on the {\imdb} dataset(1,155 items) to compare the time efficiency of using the CF method for candidate item selection with a single RTX 3090:

To analyze time efficiency, we conducted additional experiments on the {\imdb} dataset (1,155 items), comparing the performance of the CF method for candidate item selection using a single RTX 3090.
We compare two settings: \textbf{CF+\proposed}, where LightGCN selects 20 candidate items which are then re-ranked by \proposed, and \textbf{\proposed-only}, where \proposed directly ranks all items without candidate selection.
The results in Table ~\ref{tbl:computational_efficiency} show that integrating CF reduced computation time by over 98\%, highlighting the scalability and practicality of incorporating CF into our pipeline.
\input{tables/computational_efficiency}


% \begin{itemize}
% [leftmargin=*,topsep=2pt,itemsep=2pt,parsep=0pt]
%     \item \textbf{CF + \proposed}: LightGCN selected 20 candidate items, then re-ranked by \proposed.
%     \item \textbf{\proposed-only}: \proposed directly ranked all items without candidate selection.
% \end{itemize}




% \begin{table}[t]
% \centering
% \caption{Computation time comparison of CF+\proposed and \proposed-only.}
% \label{tbl:computational_efficiency}
% \resizebox{0.99\linewidth}{!}{
% \begin{tabular}{lccc}
% \toprulev
% \textbf{} & \textbf{CF} & \textbf{\proposed} & \textbf{Total time (per user)} \\
% \midrule
% CF+\proposed & 0.0019s & 7.3080s & 7.3099s \\ \midrule
% \proposed-only & - & - & 422.0396s \\
% \bottomrule
% \end{tabular}
% }
% \end{table}






==> tables/computational_efficiency.tex <==
\begin{table}
\centering
\caption{Computation time comparison of CF+\proposed and \proposed-only on {\imdb} dataset using a single RTX 3090.}
\label{tbl:computational_efficiency}
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{} & \textbf{CF} & \textbf{\proposed} & \textbf{Total time} \\
\midrule
CF+\proposed & 0.0019s & 7.3080s & 7.3099s \\ \midrule
\proposed-only & - & - & 422.0396s \\
\bottomrule
\end{tabular}
}
\end{table}
